Towards Real-world Video Face Restoration: A New Benchmark

Blind face restoration (BFR) on images has significantly progressed over the last several years, while real-world video face restoration (VFR), which is more challenging for more complex face motions such as moving gaze directions and facial orientations involved, remains unsolved. Typical BFR methods are evaluated on privately synthesized datasets or self-collected real-world low-quality face images, which are limited in their coverage of real-world video frames. In this work, we introduced new real-world datasets named FOS with a taxonomy of "Full, Occluded, and Side" faces from mainly video frames to study the applicability of current methods on videos. Compared with existing test datasets, FOS datasets cover more diverse degradations and involve face samples from more complex scenarios, which helps to revisit current face restoration approaches more comprehensively. Given the established datasets, we benchmarked both the state-of-the-art BFR methods and the video super resolution (VSR) methods to comprehensively study current approaches, identifying their potential and limitations in VFR tasks. In addition, we studied the effectiveness of the commonly used image quality assessment (IQA) metrics and face IQA (FIQA) metrics by leveraging a subjective user study. With extensive experimental results and detailed analysis provided, we gained insights from the successes and failures of both current BFR and VSR methods. These results also pose challenges to current face restoration approaches, which we hope stimulate future advances in VFR research.

==> tab/user_study_statistics_all.tex <==
\begin{tabular}{@{}c|cccccc|cc|cc@{}}
\toprule
\multicolumn{1}{l|}{} & \multicolumn{8}{c|}{FOS-real}                                                                                                                                                                                                                          & \multicolumn{2}{c}{FOS-V}                                   \\ \midrule
\multicolumn{1}{l|}{} & \multicolumn{2}{c}{F.}                                      & \multicolumn{2}{c}{O.}                                      & \multicolumn{2}{c|}{S.}                                      & \multicolumn{2}{c|}{Total}                                   & \multicolumn{2}{c}{Total}                                   \\
                     & Real.↑                       & Fidel.↑                      & Real.↑                       & Fidel.↑                      & Real.↑                       & Fidel.↑                      & Real.↑                       & Fidel.↑                      & Reconst.↑                    & Stability↑                   \\
GPEN~\cite{gpen}                 & \cellcolor[HTML]{DCE6F1}3.30 & \cellcolor[HTML]{DCE6F1}3.39 & \cellcolor[HTML]{DCE6F1}3.12 & \cellcolor[HTML]{DCE6F1}3.28 & \cellcolor[HTML]{DCE6F1}3.21 & \cellcolor[HTML]{DCE6F1}3.31 & \cellcolor[HTML]{DCE6F1}3.22 & \cellcolor[HTML]{DCE6F1}3.33 & \cellcolor[HTML]{F2DCDB}3.60 & \cellcolor[HTML]{DCE6F1}3.47 \\
GCFSR~\cite{gcfsr} & 2.91                         & \cellcolor[HTML]{DCE6F1}3.26 & 2.94                         & \cellcolor[HTML]{DCE6F1}3.23 & 2.84                         & \cellcolor[HTML]{DCE6F1}3.15 & 2.90                         & \cellcolor[HTML]{DCE6F1}3.22 & \cellcolor[HTML]{DCE6F1}3.40 & \cellcolor[HTML]{DCE6F1}3.33 \\
GFP-GAN~\cite{gfpgan}              & \cellcolor[HTML]{DCE6F1}3.05 & \cellcolor[HTML]{DCE6F1}3.22 & 2.83                         & \cellcolor[HTML]{DCE6F1}3.04 & \cellcolor[HTML]{DCE6F1}3.00 & \cellcolor[HTML]{DCE6F1}3.23 & 2.97                         & \cellcolor[HTML]{DCE6F1}3.17 & \cellcolor[HTML]{F2DCDB}3.52 & \cellcolor[HTML]{F2DCDB}3.51 \\
VQFR~\cite{vqfr}                 & \cellcolor[HTML]{DCE6F1}3.42 & \cellcolor[HTML]{DCE6F1}3.32 & 2.92                         & 2.89                         & 2.91                         & 2.85                         & \cellcolor[HTML]{DCE6F1}3.13 & \cellcolor[HTML]{DCE6F1}3.06 & 2.95                         & 2.28                         \\
RestoreFormer~\cite{restoreformer}        & 2.72                         & 2.90                         & 2.57                         & 2.83                         & 2.36                         & 2.63                         & 2.58                         & 2.80                         & \cellcolor[HTML]{DCE6F1}3.05 & 2.98                         \\
CodeFormer~\cite{codeformer}           & \cellcolor[HTML]{F2DCDB}3.64 & \cellcolor[HTML]{F2DCDB}3.64 & \cellcolor[HTML]{DCE6F1}3.43 & \cellcolor[HTML]{DCE6F1}3.47 & \cellcolor[HTML]{DCE6F1}3.29 & \cellcolor[HTML]{DCE6F1}3.31 & \cellcolor[HTML]{DCE6F1}3.48 & \cellcolor[HTML]{F2DCDB}3.50 & \cellcolor[HTML]{DCE6F1}3.19 & \cellcolor[HTML]{DCE6F1}3.46 \\
EDVR~\cite{edvr}                 & -                            & -                            & -                            & -                            & -                            & -                            & -                            & -                            & \cellcolor[HTML]{DCE6F1}3.19 & \cellcolor[HTML]{DCE6F1}3.46 \\
EDVR-GAN             & -                            & -                            & -                            & -                            & -                            & -                            & -                            & -                            & \cellcolor[HTML]{DCE6F1}3.07 & \cellcolor[HTML]{DCE6F1}3.08 \\
BasicVSR~\cite{basicvsr}             & -                            & -                            & -                            & -                            & -                            & -                            & -                            & -                            & \cellcolor[HTML]{DCE6F1}3.23 & \cellcolor[HTML]{F2DCDB}3.57 \\
BasicVSR-GAN         & -                            & -                            & -                            & -                            & -                            & -                            & -                            & -                            & 2.93                         & 2.95                         \\ \bottomrule
\end{tabular}
